From Events to Reactions: A Progress Report

Syndicate is a new coordinated, concurrent programming language. It occupies a novel point on the spectrum between the shared-everything paradigm of threads and the shared-nothing approach of actors. Syndicate actors exchange messages and share common knowledge via a carefully controlled database that clearly scopes conversations. This approach clearly simplifies coordination of concurrent activities. Experience in programming with Syndicate, however, suggests a need to raise the level of linguistic abstraction. In addition to writing event handlers and managing event subscriptions directly, the language will have to support a reactive style of programming. This paper presents event-oriented Syndicate programming and then describes a preliminary design for augmenting it with new reactive programming constructs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{D. Orchard and N. Yoshida (Eds.): Programming Language Approaches to \\ Concurrency- and Communication-Centric Software (PLACES 2016).\\
EPTCS 211, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.211.5}{10.4204/EPTCS.211.5}}
\pdfoutput=1

